Disks in Nearby Young Stellar Associations Found Via Virtual Reality

The Disk Detective citizen science project recently released a new catalog of disk candidates found by visual inspection of images from NASA's Wide-Field Infrared Survey Explorer (WISE) mission and other surveys. We applied this new catalog of well-vetted disk candidates to search for new members of nearby young stellar associations (YSAs) using a novel technique based on Gaia data and virtual reality (VR). We examined AB Doradus, Argus, $\beta$ Pictoris, Carina, Columba, Octans-Near, Tucana-Horologium, and TW Hya by displaying them in VR together with other nearby stars, color-coded to show infrared excesses found via Disk Detective. Using this method allows us to find new association members in mass regimes where isochrones are degenerate. We propose ten new YSA members with infrared excesses: three of AB Doradus (HD 44775, HD 40540 and HD 44510), one of $\beta$ Pictoris (HD 198472), two of Octans-Near (HD 157165 and BD+35 2953), and four disk-hosting members of a combined population of Carina, Columba and Tucana-Horologium: CPD-57 937, HD 274311, HD 41992, and WISEA J092521.90-673224.8. This last object (J0925) appears to be an extreme debris disk with a fractional infrared luminosity of $3.7 \times 10^{-2}$. We also propose two new members of AB Doradus that do not show infrared excesses: TYC 6518-1857-1 and CPD-25 1292. We find HD 15115 appears to be a member of Tucana-Horologium rather than $\beta$ Pictoris. We advocate for membership in Columba-Carina of HD 30447, CPD-35 525, and HD 35841. Finally, we propose that three M dwarfs, previously considered members of Tuc-Hor are better considered a separate association, tentatively called ``Smethells 165''.

==> blank.tex <==
\tablerefs{(1) \citet{2018AandA...616A...1G}. (2) This work. (3) \citet{2018ApJ...856...23G}. (4) \citet{2013ApJS..208....9P}.}
